Time-aware Random Walk Diffusion to Improve Dynamic Graph Learning

How can we augment a dynamic graph for improving the performance of dynamic graph neural networks? Graph augmentation has been widely utilized to boost the learning performance of GNN-based models. However, most existing approaches only enhance spatial structure within an input static graph by transforming the graph, and do not consider dynamics caused by time such as temporal locality, i.e., recent edges are more influential than earlier ones, which remains challenging for dynamic graph augmentation. In this work, we propose TiaRa (Time-aware Random Walk Diffusion), a novel diffusion-based method for augmenting a dynamic graph represented as a discrete-time sequence of graph snapshots. For this purpose, we first design a time-aware random walk proximity so that a surfer can walk along the time dimension as well as edges, resulting in spatially and temporally localized scores. We then derive our diffusion matrices based on the time-aware random walk, and show they become enhanced adjacency matrices that both spatial and temporal localities are augmented. Throughout extensive experiments, we demonstrate that TiaRa effectively augments a given dynamic graph, and leads to significant improvements in dynamic GNN models for various graph datasets and tasks.

==> tables/algorithm.tex <==
\vspace{-3mm}
\begin{algorithm}[t!]
    \begin{algorithmic}[1]
        \caption{\method at time $t$}
        \label{alg:method}
        \Require adjacency matrix $\A{t}$, previous time-aware diffusion matrix $\Xtilde{t-1}$, restart probability $\alpha$, time travel probability $\beta$, number $K$ of iterations, filtering threshold $\epsilon$
        \Ensure time-aware diffusion matrix $\Xtilde{t}^{\top}$
            \State $\Atilde{t} \leftarrow \mat{D}_{t}^{-1}\A{t}$ where $\mat{D}_{t} = \text{diag}$($\A{t}\vect{1}$)
            \State $\Lrwr{t} \leftarrow $ \textsc{Power-Iteration}($\Atilde{t}$, $\alpha$, $\beta$, $K$)
            \State $\S{t} \leftarrow \Lrwr{t}$  \algorithmiccomment{\textbf{Spatial augmenter}}
            \State $\T{t} \leftarrow \S{t}\Xtilde{t-1}$ \algorithmiccomment{\textbf{Temporal augmenter}}
            \State  $\X{t} \leftarrow (1 - \gamma)\S{t} + \gamma\T{t}$ where $\gamma = \beta/(\alpha + \beta)$
            \State $\Xtilde{t} \leftarrow$ filter entries of $\X{t}$ if their weights are $< \epsilon$
            \State normalize $\Xtilde{t}$ column-wise
        \State
        \Return $\Xtilde{t}^{\top}$
        \Function{Power-Iteration}{$\Atilde{t}$, $\alpha$, $\beta$, $K$}\label{alg:method:power:start}
            \State set $c \leftarrow 1 - \alpha - \beta$ and $\mat{M}_{t}^{(0)} \leftarrow \I{n}$
            \For{\text{$k \leftarrow 1$ to $K$}}
                \State $\mat{M}_{t}^{(k)} \leftarrow \I{n} + c\Atilde{t}^{\top}\mat{M}_{t}^{(k-1)}$
            \EndFor
            \State $\Lrwr{t} \leftarrow (1-c)\mat{M}_{t}^{(K)}$ where $\mat{M}_{t}^{(K)}
            \approxeq \L{t}^{-1}$
            \State normalize $\Lrwr{t}$ column-wise and \Return $\Lrwr{t}$
        \EndFunction\label{alg:method:power:end}
    \end{algorithmic}
\end{algorithm}


==> tables/datasets.tex <==
\def\arraystretch{1}
\setlength{\tabcolsep}{4.8pt}
\begin{table}[t!]
    \vspace{-2mm}
    \captionsetup{font=small}
    \caption{
        Summary of datasets. $n$ and $m$ are the total numbers of nodes and edges, resp.
        $T$ and $L$ are the numbers of time steps and labels, resp.
        $\bar{n}_t$ and $\bar{m}_t$ are the average numbers of activated nodes and edges over time, resp.
        $\bar{C}_{t} = \bar{m}_{t}/\bar{n}_t$.
        The first 3 data are used for link prediction, and the others are for node classification.
    }
    \label{tab:data}
    \small
    \begin{tabular}{lrrrrrr}
        \hline
        \toprule
        \textbf{Datasets} & \multicolumn{1}{r}{$n$} & \multicolumn{1}{r}{$m$} & \multicolumn{1}{r}{$T$} & \multicolumn{1}{r}{$L$} & \multicolumn{1}{r}{$\lfloor\bar{n}_{t}\rfloor$} & \multicolumn{1}{r}{$\bar{C}_{t}$} \\
        \midrule
        \textbf{BitcoinAlpha} & 3,783 & 31,748 & 138 & 2 & 105 & 2.2 \\
        \textbf{WikiElec} & 7,125 & 212,854 & 100 & 2 & 354 & 6.0 \\
        \textbf{RedditBody} & 35,776 & 484,460 & 88 & 2 & 2,465 & 2.2 \\
        \midrule
        \textbf{Brain} & 5,000 & 1,955,488 & 12 & 10 & 5,000 & 32.6 \\
        \textbf{DBLP-3} & 4,257 & 23,540 & 10 & 3 & 782 & 3.0 \\
        \textbf{DBLP-5} & 6,606 & 42,815 & 10 & 5 & 1,212 & 3.5 \\
        \textbf{Reddit} & 8,291 & 264,050 & 10 & 4 & 2,071 & 12.8 \\
        \bottomrule
        \hline
    \end{tabular}
    \vspace{-1mm}
\end{table}


==> tables/link_auc.tex <==
\def\arraystretch{0.9}
\setlength{\tabcolsep}{2.4pt}
\begin{table*}[t!]
\vspace{-1mm}
\begin{threeparttable}[t]
    \caption{
        \label{tab:link_auc}
        Temporal link prediction accuracy (AUC) where \textsc{None} is a result without augmentation, and {\color{red}$\blacktriangle$} (or {\color{blue}$\blacktriangledown$}) indicates improvement (or degradation) compared to None. 
        \method shows consistent improvement across most models and datasets.
    }
    \begin{tabular}{@{}cccccccccc@{}}
        \hline
        \toprule
        \multirow{2}[2]{*}{\textbf{AUC}} & \multicolumn{3}{c}{\textbf{BitcoinAlpha}} & \multicolumn{3}{c}{\textbf{WikiElec}} & \multicolumn{3}{c}{\textbf{RedditBody}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
        & \textbf{GCN} & \textbf{GCRN} & \textbf{EGCN} & \textbf{GCN} & \textbf{GCRN} & \textbf{EGCN} & \textbf{GCN} & \textbf{GCRN} & \textbf{EGCN} \\
        \midrule
        \textsc{None} & \lwt57.3±1.6\lwt & \lwt80.3±6.0\lwt & \lwt58.8±1.1\lwt & \lwt59.9±0.9\lwt & \lwt72.1±2.4\lwt & \lwt66.9±3.7\lwt & \lwt77.6±0.4\lwt & \lwt88.9±0.3\lwt & \lwt77.6±0.2\lwt \\
        \midrule
        \textsc{DropEdge} & \lbt56.3±1.0\lwt & \lbt73.9±2.2\lwt & \lbt57.4±0.9\lwt & \lbt50.1±1.0\lwt & \lbt56.0±9.3\lwt & \lbt47.9±6.4\lwt & \lbt73.0±0.4\lwt & \lbt77.0±1.7\lwt & \lbt71.9±0.7\lwt \\
        \textsc{GDC} & \lrt57.5±1.6\lwt & \lbt77.3±6.5\lwt & \lbt57.4±1.2\lwt & \lrt62.8±0.8\lwt & \lbt67.9±1.0\lwt & \lbt63.1±0.7\lwt & \lbt74.6±0.0\lwt & \lbt86.4±0.3\lwt & \lbt73.8±0.3\lwt \\
        \textsc{Merge} & \lrt66.8±2.6\lwt & \lrt93.1±0.4\lwt & \lrt61.0±9.2\lwt & \lrt60.6±1.7\lwt & \lbt68.4±3.2\lwt & \lbt60.7±1.3\lwt & \lbt69.7±0.7\lwt & \lrt{89.8±0.5}\lwt & \lrt80.3±0.5\lwt \\
        \midrule
        \method & \lrt\textbf{76.0±1.3}\lwt & \lrt\textbf{94.6±0.8}\lwt & \lrt\textbf{77.2±1.4}\lwt & \lrt\textbf{69.0±1.2}\lwt & \lrt\textbf{73.4±2.2}\lwt & \lrt\textbf{69.1±0.3}\lwt & \lrt\textbf{80.8±0.6}\lwt & \lrt\textbf{90.2±0.4}\lwt & \lrt\textbf{82.0±0.1}\lwt \\
        \bottomrule
        \hline
    \end{tabular}
\end{threeparttable}
\vspace{-2mm}
\end{table*}


==> tables/node_f1.tex <==
\def\arraystretch{1.1}
\setlength{\tabcolsep}{0.8pt}
\begin{table*}[t!]
\vspace{-2mm}
\small
\begin{threeparttable}[t]
    \caption{
        \label{tab:node_f1}
        Node classification accuracy (Macro F1-score) where \textsc{None} is a result without augmentation, and {\color{red}$\blacktriangle$} (or {\color{blue}$\blacktriangledown$}) indicates improvement (or degradation) compared to None.
        \method shows consistent improvement across most models and datasets.
    }
    \begin{tabular}{@{}ccccccccccccc@{}}
        \hline
        \toprule
        \multirow{2}[2]{*}{\textbf{Macro F1}} & \multicolumn{3}{c}{\wt\textbf{Brain}} & \multicolumn{3}{c}{\wt\textbf{Reddit}} & \multicolumn{3}{c}{\wt\textbf{DBLP-3}} & \multicolumn{3}{c}{\wt\textbf{DBLP-5}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
        & \wt\textbf{GCN} & \wt\textbf{GCRN} & \wt\textbf{EGCN} & \wt\textbf{GCN} & \wt\textbf{GCRN} & \wt\textbf{EGCN} & \wt\textbf{GCN} & \wt\textbf{GCRN} & \wt\textbf{EGCN} & \wt\textbf{GCN} & \wt\textbf{GCRN} & \wt\textbf{EGCN} \\
        \midrule
        \textsc{None} & \wt44.7±0.8 & \wt66.8±1.0 & \wt43.4±0.7 & \wt18.2±2.9 & \wt40.4±1.6 & \wt18.6±2.3 & \wt53.4±2.6 & \wt83.1±0.6 & \wt51.3±2.7 & \wt69.6±0.9 & \wt75.4±0.7 & \wt68.5±0.6 \\
        \midrule
        \textsc{DropEdge} & \bt35.2±1.7 & \rt67.8±0.6 & \bt39.7±1.8 & \rt\textbf{19.4±0.8} & \bt40.3±1.4 & \bt{18.0±2.7} & \rt55.8±1.9 & \rt84.3±0.6 & \rt52.4±1.7 & \rt70.5±0.5 & \rt75.6±0.7 & \bt68.0±0.7 \\
        \textsc{GDC} & \rt63.2±1.2 & \rt88.0±1.5 & \rt67.3±1.3 & \bt17.5±2.3 & \rt41.0±1.6 & \bt18.5±2.8 & \rt53.4±2.1 & \rt84.7±0.5 & \rt52.8±2.2 & \rt70.0±0.7 & \rt75.5±1.2 & \rt69.1±1.0 \\
        \textsc{Merge} & \bt34.4±3.4 & \bt63.2±1.6 & \rt53.0±0.9 & \rt19.3±3.0 & \bt39.6±0.8 & \rt 20.4±3.0 & \rt54.9±3.1 & \bt83.0±1.4 & \rt53.3±1.2 & \rt{70.8±0.4} & \bt74.5±0.8 & \rt69.7±1.6 \\
        \midrule
        \textbf{\method} & \rt\textbf{68.7±1.2} & \rt\textbf{91.3±1.0} & \rt\textbf{72.0±0.6} & \rt{18.4±3.0} & \rt\textbf{41.5±1.5} & \rt\textbf{21.9±1.6} & \rt\textbf{57.5±2.2} & \rt\textbf{84.9±1.6} & \rt\textbf{56.4±1.8} & \rt{\textbf{71.1±0.6}} & \rt\textbf{77.9±0.4} & \rt\textbf{70.1±1.0} \\
        \bottomrule
        \hline
    \end{tabular}
\end{threeparttable}
\end{table*}

